Particle formation in oxymethylene ethers (OMEn, n = 2-4) / ethylene premixed flames

Alternative synthetic fuels can be produced by renewable energy sources and represent a potential route for solving long-term energy storage. Among them, oxygenated fuels have the advantage of significantly reducing pollutant emissions and can therefore be used as carbon-neutral substitute fuels for transportation. In this work, the sooting propensity of different oxymethylene ethers (OMEn) is investigated using a combined experimental and numerical study on a series of burner-stabilized premixed flames under mild to severe sooting conditions. Herein, mixtures of ethylene in combination with the three individual OMEn for n=2-4 are compared in terms of soot formation behavior with pure ethylene flames. The kinetic mechanism from Sun et al. (Proc. Combust. Inst. 36, 1269-1278, 2017) for oxymethylene ether OMEn combustion with n=1-3 is extended to include OME4 decomposition and combustion kinetics. In the numerical simulations, the kinetic mechanism is combined with a detailed quadvariate soot model which uses the Conditional Quadrature Method of Moments and validated with Laser-Induced Fluorescence (LIF) and Laser-Induced Incandescence (LII) measurements. It is observed, that the three investigated OMEn with n=2-4 show similar sooting behavior, mainly reducing larger aggregates while not significantly affecting the formation of smaller particles. Furthermore, the extent of soot reduction is comparable among the three OMEn. The trends and overall reduction are very well captured by the model. The modeling results are analyzed through reaction path analyses and sensitivity studies which show the important role of OMEn decomposition and the formation of CH2O under these rich conditions to reduce species relevant for soot formation. This is at the base of the negligible observed differences in terms of soot formation for the different OMEn fuels.

==> parts/mechanism.tex <==
\begin{table*}[h!] \small
\caption{ Selected reactions of the \ce{OME4} sub-mechanism derived from the \ce{OME3} mechanism from Sun et al.~\cite{Sun2017}. Reaction rate expression is $k=A T^n \mathrm{exp}(-E_a/RT)$.  Units are expressed in s$^{-1}$, cm$^3$ and cal/mol.}
\small{
\centerline{\begin{tabular}{llcccccc}
\hline 
No. & Reaction & {} & {} $A$ & $n$ & E_a \\
\hline
1 & DMM4+M = COCOCOCOCOj+CH3+M   &     &   2.33E+19  & -0.66   & 84139.5   \\ %    ! analogy to the reaction CH3OCH3=CH3+CH3O from Reference 1
 &    &LOW                               &    /1.72E+59  & -11.40  &  93295.6/  \\ %
 &              &             TROE        &   /1.0      &  1.0E-30  &  880./    \\ %
 &  \multicolumn{5}{r}{H2/3.0/ H2O/9.0/ CH4/3.0/ CO/2.25/ CO2/3.0/ C2H6/4.5/ Ar/1.0} \\%     ! analogy to the reaction CH3CH2OCH2CH3=CH3CH2O+CH3CH2 from reference 2
2 &   DMM4+M = DMM3A+M+CH3O        & {}   &  1.24E+25  &  -2.29  &  85330.    \\
 &    & {}LOW                                &  /3.55E+83  & -18.70 &   98640/   \\
 &    & {}TROE                               &   /9.0E-6 &  506  &  1.14E+10  {}   2470/  \\ %    ! analogy to the reaction CH3CH2OCH2CH3=CH3CH2O+CH3CH2 from reference 2
3 & DMM4+M = COCOCOCOj+CH3OCH2+M   & {}   &  1.24E+25  &  -2.29 &   85330.   \\
 &  & {}  LOW                                &  /3.55E+83  & -18.70  &  98640/    \\
 &   & {} TROE                                &    /9.0E-6 &  506  & 1.14E+10 {}  2470/    \\%    ! analogy to the reaction CH3CH2OCH2CH3=CH3CH2O+CH3CH2 from reference 2
4 & DMM4+M = DMM2A+CH3OCH2O+M  & {}        &        1.24E+25 &   -2.29 &   85330.     \\%
 &   & {}LOW                                 &       /3.55E+83 &  -18.70 &   98640/      \\
 &   & {}TROE                                &     /9.0E-6     &  506    & 1.14E+10 {} 2470/\\%
5 & DMM4+M = DMM3+CH2O+M    & {}          &     1.0E+14     &   0.00  &  65210.      \\%     ! analogy to the reaction CH3CH2OCH2CH3=CH3CH2OH+C2H4 from reference 2
 & & {}LOW                                   &    /5.72E+96    &  -23.0  &  80813 /      \\
 & & {} TROE                                  &    /1.17E-3     &  379    & 1.58E+7 {}  4730/\\%
% & !hydrogen abstractions and b-scissions
6 & DMM4+H = DMM4A+H2      & {}                 &  3.940E+00 &   4.13 &   1.780E+03  \\  % ! analogy to the reaction CH3OCH3+H=CH3OCH2+H2 from Reference 1
7 & DMM4+H = DMM4B+H2     & {}                  &  7.400E+14 &   0.00 &   3.170E+03  \\  % ! analogy to the reaction CH3CH2OCH2CH3+H=CH3CH2OCHCH3+H2 from Reference 2
8 & DMM4+H = DMM4C+H2     & {}                  &  3.700E+14 &   0.00 &   3.170E+03  \\  % ! analogy to the reaction CH3CH2OCH2CH3+H=CH3CH2OCHCH3+H2 from Reference 2, with the A factor divided by 2
9 & DMM4+OH = DMM4A+H2O   & {}                  &  1.954E+07 &   1.89 &  -3.656E+02  \\  % ! analogy to the reaction CH3OCH3+OH=CH3OCH2+H2O from Reference 3
10 & DMM4+OH = DMM4B+H2O      & {}               &  2.260E+03 &   2.93 &   4.040E+03  \\  % ! analogy to the reaction CH3CH2OCH2CH3+OH=CH3CH2OCHCH3+H2O from Reference 3
11 & DMM4+OH = DMM4C+H2O       & {}              &  1.130E+03 &   2.93 &   4.040E+03  \\  % ! analogy to the reaction CH3CH2OCH2CH3+OH=CH3CH2OCHCH3+H2O from Reference 3, with the A factor divided by 2
12 & DMM4+O = DMM4A+OH          & {}             &  2.689E+07 &   2.00 &   2.632E+03  \\  % ! analogy to the reaction CH3CH2OCH2CH3+O=CH3CH2OCH2CH2+OH from Reference 4
13 & DMM4+O = DMM4B+OH              & {}         &  1.600E+13 &   0.00 &   3.038E+03  \\  % ! analogy to the reaction CH3CH2OCH2CH3+O=CH3CH2OCHCH3+OH from Reference 5
15 & DMM4+O = DMM4C+OH                  & {}     &  8.000E+12 &   0.00 &   3.038E+03  \\  % ! analogy to the reaction CH3CH2OCH2CH3+O=CH3CH2OCHCH3+OH from Reference 5, with the A factor divided by 2
16 & DMM4+CH3 = DMM4A+CH4               & {}     &  1.019E+01 &   3.78 &   9.688E+03  \\  % ! analogy to the reaction CH3OCH3+CH3=CH3OCH2+CH4 from Reference 6
17 & DMM4+CH3 = DMM4B+CH4               & {}     &  9.993E+11 &   0.00 &   9.767E+03  \\  % ! analogy to the reaction CH3CH2OCH2CH3+CH3=CH3CH2OCHCH3+CH4 from Reference 7
18 & DMM4+CH3 = DMM4C+CH4               & {}     &  4.997E+11 &   0.00 &   9.767E+03  \\  % ! analogy to the reaction CH3CH2OCH2CH3+CH3=CH3CH2OCHCH3+CH4 from Reference 7,with the A factor divided by 2
19 & DMM4+HO2 = DMM4A+H2O2          & {}         &  1.680E+03 &   0.00 &   1.769E+04  \\  % ! analogy to the reaction CH3OCH3+HO2=CH3OCH2+H2O2 from Reference 8
20 & DMM4+HO2 = DMM4B+H2O2              & {}     &  2.950E+04 &   2.60 &   1.390E+04  \\  % ! analogy to the reaction CH3OCH2OCH3+HO2=CH3OCHOCH3+H2O2 from Reference 9,with the A factor multiplied by 2
21 & DMM4+HO2 = DMM4C+H2O2              & {}     &  1.475E+04 &   2.60 &   1.390E+04  \\  % ! analogy to the reaction CH3OCH2OCH3+HO2=CH3OCHOCH3+H2O2 from Reference 9
22 & DMM4+O2 = DMM4A+HO2                & {}     &  2.000E+13 &   0.00 &   4.560E+04  \\  % ! analogy to the reaction CH3OCH2OCH3+O2=CH3OCH2OCH2+HO2 from Reference 9
23 & DMM4+O2 = DMM4B+HO2                & {}     &  6.660E+12 &   0.00 &   4.354E+04  \\  % ! analogy to the reaction CH3OCH2OCH3+O2=CH3OCHOCH3+HO2 from Reference 9, with the A factor multiplied by 2
24 & DMM4+O2 = DMM4C+HO2            & {}         &  3.330E+12 &   0.00 &   4.354E+04  \\  % ! analogy to the reaction CH3OCH2OCH3+O2=CH3OCHOCH3+HO2 from Reference 9
25 & DMM4+CH3O = DMM4A+CH3OH        & {}         &  6.020E+11 &   0.00 &   4.074E+03  \\  % ! analogy to the reaction CH3OCH3+CH3O=CH3OCH2+CH3OH from Reference 8
26 & DMM4+CH3O = DMM4B+CH3OH        & {}         &  1.000E+12 &   0.00 &   4.552E+03  \\  % ! analogy to the reaction CH3OCH2CH3+CH3O=CH3OCHOCH3+CH3OH from Reference 9, with the A factor multiplied by 2
27 & DMM4+CH3O = DMM4C+CH3OH        & {}         &  5.000E+11 &   0.00 &   4.552E+03  \\  % ! analogy to the reaction CH3OCH2CH3+CH3O=CH3OCHOCH3+CH3OH
28 & DMM4A = DMM3A+CH2O                 & {}     &  4.450E+14 &  -0.22 &   2.727E+04  \\  % ! analogy to the reaction CH3OCH2=CH3+CH2O from Reference 10
29 & DMM4B = COCOCOCOC*O+CH3            & {}     &  2.860E+15 &  -0.24 &   1.017E+04  \\  % ! analogy to the reaction CH3CH2OCHCH3=CH3HCO+CH3OCH2 from Reference 2
30 & DMM4B = DMM2A+CH3OCHO              & {}     &  2.860E+15 &  -0.24 &   1.017E+04  \\  % ! analogy to the reaction CH3CH2OCHCH3=CH3HCO+CH3OCH2 from Reference 2
31 & DMM4C = COCOCOC*O+CH3OCH2          & {}     &  5.720E+15 &  -0.24 &   1.017E+04  \\  % ! analogy to the reaction CH3CH2OCHCH3=CH3HCO+CH3OCH2 from Reference 2, with the A factor multiplied by 2

\iffalse
 & COCOCOCOCOj = CH2O+COCOCOCOj          & {}  &  1.570E+21 &  -2.44 &   1.684E+04  \\  % ! analogy to the reaction CH3CH2CH2CH2O=CH3CH2CH2+CH2O from Reference 11
 & COCOCOCOCOj = H+COCOCOCOC*O           & {}  &  8.890E+10 &   0.75 &   2.106E+04  \\  % ! analogy to the reaction CH3CH2CH2O=CH3CH2HCO+H from Reference 11
%  & !secondary mech for COCOCOCOC*O
 & COCOCOCOC*O+H = CjOCOCOCOC*O+H2  & {}       &  1.880E+05 &   2.80 &   6.280E+03  \\  % ! analogy to the reaction CH3CH2OCHO+H=CH2CH2OCHO+H2 from Reference 12
 & COCOCOCOC*O+H = COCjOCOCOC*O+H2  & {}       &  1.880E+05 &   2.80 &   6.280E+03  \\  % ! analogy to the reaction CH3CH2OCHO+H=CH2CH2OCHO+H2 from Reference 12
 & COCOCOCOC*O+H = COCOCjOCOC*O+H2  & {}       &  3.250E+05 &   2.40 &   4.471E+03  \\  % ! analogy to the reaction CH3CH2OCHO+H=CH3HCOCHO+H2 from Reference 12
 & COCOCOCOC*O+H = COCOCOCjOC*O+H2      & {}   &  3.250E+05 &   2.40 &   4.471E+03  \\  % ! analogy to the reaction CH3CH2OCHO+H=CH3HCOCHO+H2 from Reference 12
 & COCOCOCOC*O+H = COCOCOCOCj*O+H2       & {}  &  6.500E+05 &   2.40 &   4.471E+03  \\  % ! analogy to the reaction CH3CH2OCHO+H=CH2HCOCHO+H2 from Reference 12
 & COCOCOCOC*O+OH = CjOCOCOCOC*O+H2O       &  1.050E+05 &   1.00 &   1.586E+03  \\  % ! analogy to the reaction CH3CH2OCHO+OH=CH2CH2OCHO+H2O from Reference 12
 & COCOCOCOC*O+OH = COCjOCOCOC*O+H2O     & {}  &  1.050E+05 &   1.00 &   1.586E+03  \\  % ! analogy to the reaction CH3CH2OCHO+OH=CH2CH2OCHO+H2O from Reference 12
 & COCOCOCOC*O+OH = COCOCjOCOC*O+H2O    & {}   &  1.160E+07 &   1.60 &  -3.500E+01  \\  % ! analogy to the reaction CH3CH2OCHO+OH=CH3HCOCHO+H2O from Reference 12
 & COCOCOCOC*O+OH = COCOCOCjOC*O+H2O     & {}  &  1.160E+07 &   1.60 &  -3.500E+01  \\  % ! analogy to the reaction CH3CH2OCHO+OH=CH3HCOCO+OH2O from Reference 12
 & COCOCOCOC*O+OH = COCOCOCOCj*O+H2O     & {}  &  2.330E+07 &   1.60 &  -3.500E+01  \\  % ! analogy to the reaction CH3CH2OCHO+OH=CH2CH2OCO+H2O from Reference 12
 & COCOCOCOC*O+O = CjOCOCOCOC*O+OH       & {}  &  1.030E+14 &   0.00 &   7.850E+03  \\  % ! analogy to the reaction CH3CH2OCHO+O=CH2CH2OCHO+OH from Reference 12
 & COCOCOCOC*O+O = COCjOCOCOC*O+OH       & {}  &  1.030E+14 &   0.00 &   7.850E+03  \\  % ! analogy to the reaction CH3CH2OCHO+O=CH2CH2OCHO+OH from Reference 12
 & COCOCOCOC*O+O = COCOCjOCOC*O+OH       & {}  &  2.810E+13 &   0.00 &   5.200E+03  \\  % ! analogy to the reaction CH3CH2OCHO+O=CH3HCOCHO+OH from Reference 12
 & COCOCOCOC*O+O = COCOCOCjOC*O+OH       & {}  &  2.810E+13 &   0.00 &   5.200E+03  \\  % ! analogy to the reaction CH3CH2OCHO+O=CH3HCOCHO+OH from Reference 12
 & COCOCOCOC*O+O = COCOCOCOCj*O+OH        & {} &  5.510E+05 &   2.50 &   2.830E+03  \\  % ! analogy to the reaction CH3CH2OCHO+O=CH3CH2OCO+OH from Reference 12
 & COCOCOCOC*O+CH3 = CjOCOCOCOC*O+CH4    & {}  &  1.290E+12 &   0.00 &   1.160E+04  \\  % ! analogy to the reaction CH3CH2OCHO+CH3=CH2CH2OCHO+CH4 from Reference 12
 & COCOCOCOC*O+CH3 = COCjOCOCOC*O+CH4     & {} &  1.290E+12 &   0.00 &   1.160E+04  \\  % ! analogy to the reaction CH3CH2OCHO+CH3=CH2CH2OCHO+CH4 from Reference 12
 & COCOCOCOC*O+CH3 = COCOCjOCOC*O+CH4    & {}  &  3.980E+11 &   0.00 &   9.500E+03  \\  % ! analogy to the reaction CH3CH2OCHO+CH3=CH3HCOCHO+CH4 from Reference 12
 & COCOCOCOC*O+CH3 = COCOCOCjOC*O+CH4    & {}  &  3.980E+11 &   0.00 &   9.500E+03  \\  % ! analogy to the reaction CH3CH2OCHO+CH3=CH3HCOCHO+CH4 from Reference 12
 & COCOCOCOC*O+CH3 = COCOCOCOCj*O+CH4    & {}  &  1.510E+00 &   3.50 &   5.481E+03  \\  % ! analogy to the reaction CH3CH2OCHO+CH3=CH3CH2OCO+CH4 from Reference 12
 & COCOCOCOC*O+HO2 = CjOCOCOCOC*O+H2O2   & {}  &  1.680E+13 &   0.00 &   2.043E+04  \\  % ! analogy to the reaction CH3CH2OCHO+HO2=CH2CH2OCHO+H2O2 from Reference 12
 & COCOCOCOC*O+HO2 = COCjOCOCOC*O+H2O2   & {}  &  1.680E+13 &   0.00 &   2.043E+04  \\  % ! analogy to the reaction CH3CH2OCHO+HO2=CH2CH2OCHO+H2O2 from Reference 12
 & COCOCOCOC*O+HO2 = COCOCjOCOC*O+H2O2   & {}  &  5.600E+12 &   0.00 &   1.770E+04  \\  % ! analogy to the reaction CH3CH2OCHO+HO2=CH3HCOCHO+H2O2 from Reference 12
 & COCOCOCOC*O+HO2 = COCOCOCjOC*O+H2O2   & {}  &  5.600E+12 &   0.00 &   1.770E+04  \\  % ! analogy to the reaction CH3CH2OCHO+HO2=CH3HCOCHO+H2O2 from Reference 12
 & COCOCOCOC*O+HO2 = COCOCOCOCj*O+H2O2   & {}  &  9.640E+03 &   2.60 &   1.391E+04  \\  % ! analogy to the reaction CH3CH2OCHO+HO2=CH3CH2OCO+H2O2 from Reference 12
 & COCOCOCOC*O+O2 = CjOCOCOCOC*O+HO2     & {}  &  2.000E+13 &   0.00 &   4.750E+04  \\  % ! analogy to the reaction CH3CH2OCHO+O2=CH2CH2OCHO+HO2 from Reference 12
 & COCOCOCOC*O+O2 = COCjOCOCOC*O+HO2     & {}  &  2.000E+13 &   0.00 &   4.750E+04  \\  % ! analogy to the reaction CH3CH2OCHO+O2=CH2CH2OCHO+HO2 from Reference 12
 & COCOCOCOC*O+O2 = COCOCjOCOC*O+HO2     & {}  &  4.000E+13 &   0.00 &   4.750E+04  \\  % ! analogy to the reaction CH3CH2OCHO+O2=CH3HCOCHO+HO2 from Reference 12
 & COCOCOCOC*O+O2 = COCOCOCjOC*O+HO2     & {}  &  4.000E+13 &   0.00 &   4.750E+04  \\  % ! analogy to the reaction CH3CH2OCHO+O2=CH3HCOCHO+HO2 from Reference 12
 & COCOCOCOC*O+O2 = COCOCOCOCj*O+HO2     & {}  &  2.000E+13 &   0.00 &   4.970E+04  \\  % ! analogy to the reaction CH3CH2OCHO+O2=CH3CH2OCO+HO2 from Reference 12
 & COCOCOCOC*O+CH3O = CjOCOCOCOC*O+CH3OH  & {} &  3.000E+11 &   0.00 &   7.000E+03  \\  % ! analogy to the reaction CH3CH2OCHO+CH3O=CH2CH2OCHO+CH3OH from Reference 12
 & COCOCOCOC*O+CH3O = COCjOCOCOC*O+CH3OH & {}  &  3.000E+11 &   0.00 &   7.000E+03  \\  % ! analogy to the reaction CH3CH2OCHO+CH3O=CH2CH2OCHO+CH3OH from Reference 12
 & COCOCOCOC*O+CH3O = COCOCjOCOC*O+CH3OH  & {} &  3.000E+11 &   0.00 &   7.000E+03  \\  % ! analogy to the reaction CH3CH2OCHO+CH3O=CH3HCOCHO+CH3OH from Reference 12
 & COCOCOCOC*O+CH3O = COCOCOCjOC*O+CH3OH  & {} &  3.000E+11 &   0.00 &   7.000E+03  \\  % ! analogy to the reaction CH3CH2OCHO+CH3O=CH3HCOCHO+CH3OH from Reference 12
 & COCOCOCOC*O+CH3O = COCOCOCOCj*O+CH3OH  & {} &  5.480E+11 &   0.00 &   5.000E+03  \\  % ! analogy to the reaction CH3CH2OCHO+CH3O=CH3HCOCHO+CH3OH from Reference 12
 & CjOCOCOCOC*O = CjOCOCOC*O+CH2O         & {} &  1.340E+13 &  -0.40 &   2.461E+04  \\  % ! analogy to the reaction CH2CH2OCHO=C2H4+OCHO from Reference 12
 & COCjOCOCOC*O = CH3OCH2OCHO+CH2OCHO     & {} &  4.170E+15 &  -0.90 &   1.404E+04  \\  % ! analogy to the reaction CH3HCOCHO=CH3HCO+CHO from Reference 12
 & COCOCjOCOC*O = CH3OCH2OCHO+CH2OCHO     & {} &  4.170E+15 &  -0.90 &   1.404E+04  \\  % ! analogy to the reaction CH3HCOCHO=CH3HCO+CHO from Reference 12
 & COCOCOCjOC*O = COCOCOC*O+HCO          & {}  &  4.170E+15 &  -0.90 &   1.404E+04  \\  % ! analogy to the reaction CH3HCOCHO=CH3HCO+CHO from Reference 12
 & COCOCOCOCj*O = DMM2A+CO2              & {}  &  1.89E+09  &   0.13 &   7974.3     \\  % ! analogy to the reaction CH3OCO=CH3+CO2 from Reference 13
 & COCOCOCOCj*O = COCOCOCOj+CO           & {}  &  6.11E-02  &   2.95 &   17750.1    \\  % ! analogy to the reaction CH3OCO=CH3+CO2 from Reference 13
\fi


\hline
\end{tabular}}
}

Note: 
DMM4: \ce{CH3OCH2OCH2OCH2OCH2OCH3}; 
DMM4A: \ce{CH3OCH2OCH2OCH2OCH2OCH2}; 
DMM4B: \ce{CH3OCH2OCH2OCH2OCHOCH3}; 
DMM4C: \ce{CH3OCH2OCH2OCHOCH2OCH3};
DMM3: \ce{CH3OCH2OCH2OCH2OCH3};
DMM3A: \ce{CH3OCH2OCH2OCH2OCH2};
DMM2A: \ce{CH3OCH2OCH2OCH2};
COCOCOCOCOj:  \ce{CH3OCH2OCH2OCH2OCH2O};
COCOCOCOj:  \ce{CH3OCH2OCH2OCH2O};
COCOCOCOC*O: \ce{CH3OCH2OCH2OCH2OCHO};
COCOCOC*O: \ce{CH3OCH2OCH2OCHO}.

\label{Tab:mechanism}
\end{table*}


